Speedster: A TEE-assisted State Channel System

State channel network is the most popular layer-2 solution to theissues of scalability, high transaction fees, and low transaction throughput of public Blockchain networks. However, the existing works have limitations that curb the wide adoption of the technology, such as the expensive creation and closure of channels, strict synchronization between the main chain and off-chain channels, frozen deposits, and inability to execute multi-party smart contracts. In this work, we present Speedster, an account-based state-channel system that aims to address the above issues. To this end, Speedster leverages the latest development of secure hardware to create dispute-free certified channels that can be operated efficiently off the Blockchain. Speedster is fully decentralized and provides better privacy protection. It supports fast native multi-party contract execution, which is missing in prior TEE-enabled channel networks. Compared to the Lightning Network, Speedster improves the throughput by about 10,000X and generates 97% less on-chain data with a comparable network scale.

==> paragraphs/figure/Ideal_Channel.tex <==
\begin{figure}[htbp]
\begin{framed}

\begin{center}
  
\text{$\mathcal{F}_{channel}$[$\ell$, $\mathcal{P}_L$, $\mathcal{P}_R]$}: 

\end{center}

\noindent \textbf{Initially:}
%  $sk \xleftarrow{\text{\$}} \{ 0, 1\}^\lambda  $
% $Recv := \perp, 
 $Cert := \emptyset, \state := \overrightarrow{0}, r := 0, cid \sample \bin^*$

\bigskip

\noindent \textbf{On receive}( 'authenticate', $cert_b$) from $\mathcal{P}_b$ where $b \in \{L,R \}$: 

assert $ Cert[b] = \perp$ 

$Cert[b] := cert_b$

Send ($\mathcal{P}_b$, $\mathcal{P}_{\neg b}$, 'authenticate', $\ell$($cert_b$)) to $\adv$;



await 'OK' from $\adv$

send('authenticate', cert) to $\mathcal{P}_{\neg b}$

\bigskip

\noindent \textbf{On receive}('send',$inp$) from $\mathcal{P}_b$ where $b \in \{L,R \}$:

assert $Cert[b] \neq \perp$

% $\$val, _$ := parse($inp$)

$(\state', outp) := Contract_{cid}(\mathcal{P}_b, \state, inp)$

$msg := (\mathcal{P}_b\concat r\concat inp\concat \state'\concat outp)$

leak ($\mathcal{P}_b$, $\ell(msg)$) to $\adv$; await 'OK' from $\adv$

send('receive',$msg$) to $\mathcal{P}_{\neg b}$

\bigskip

\textbf{On receive 'send' from both participants at round r:}

$\state := \state'$

$r := r+1$

\bigskip


\noindent \textbf{On receive}('claim') from $\mathcal{P}_b$ where $b \in \{L,R \}$:

assert $Cert[\neg b] \neq \perp$

send($Cert[\neg b], state$) to $\mathcal{P}_b$

\end{framed}
\label{fig:Ideal_channel}
 \caption{Ideal certified channel functionality of \TheName{}. $\ell$ denotes the leakage function.} 
\end{figure}

==> paragraphs/figure/Ideal_State.tex <==
% \begin{algorithm}
 
% \noindent \textbf{Initially:}

% % $\forall i \forall j \mathcal{F}^{i \leftrightarrow j}_{channel} \neq \perp$ where $i,j \in [N]$ and $i \neq j$

% $ci^{TEE}_{id} \xleftarrow{\text{\$}} \{ 0, 1\}^\lambda $,
%  $sk := \mathcal{H}(ci^{TEE}_{id}) $

% \bigskip


% \noindent \textbf{On receive}($'join', x_i,ci_{id} $) from $\mathcal{P}_i$:

% % assert $\mathcal{F}^i_{channel}$

% assert $ci^{TEE}_{id} = ci_{id} $

% assert $\mathcal{P}_i$ has never join before

% $sk := \mathcal{H}(sk||x_i) $ 

% leak($\mathcal{P}_i, \mid 'join'\parallel x_i \parallel ci_{id} \mid$) to $\mathcal{A}$; await until receive 'OK' from $\mathcal{A}$

% Send($'join',x_i,ci_{id}$) to other participants

% \bigskip

% \noindent \textbf{On receive}($'trans', inp_i,ci_{id} $) from $\mathcal{P}_i$:

% assert $ci^{TEE}_{id} = ci_{id} $

% $(outp,st') := \mathcal{C}(inp_i,st)$

% $ct :=\mathcal{AE}.Enc(sk,inp,st',ci_{id}) $

% $st := st'$

% leak ($\mathcal{P}_i,ci_{id},ct$) to $\mathcal{A}$. await 'OK' from $\mathcal{A}$

% output($ci_{id},outp$)

% send($'trans',ci_{id},ct$) to other participants

% \bigskip

% \caption{\text{$\mathcal{F}_{mpsc}[\mathcal{C},\mathcal{P}_1, \mathcal{P}_1, \mathcal{P}_2, ... ,\mathcal{P}_N]$}: Ideal functionality of Multi-party State Channel(mpsc) in \TheName{} system.}

% \label{fig:Ideal_state}

% \end{algorithm}

==> paragraphs/figure/comtable2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%  of one target node with n participants in a topology as shown in Figure~\ref{fig:star_topology}. $\aveChannel{}$ is the number of average channel for each node; p is the size of committee in TeeChain and SFMC and m is the minimum committee signatures required
\begin{table*}[t]
 \centering
\caption{Number of on-chain transactions and Blockchain costs (BC) for each channel under unilateral.}
\footnotesize
\label{tab:blockchaincost2}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Payment Channel\end{tabular}}} & \multicolumn{2}{c}{\textbf{Setup}} & \multicolumn{2}{c}{\textbf{Open Channel}} & \multicolumn{2}{c}{\textbf{Close Channel}} & \multicolumn{2}{c}{\textbf{Claim}} & \multicolumn{2}{c}{\textbf{Total}} \\ \cmidrule(l){2-11}
 & No.tx & BC & No.tx & BC & No.tx & BC & No.tx & BC & No.tx & BC \\ \midrule

LN~\cite{lnd} & 2 & 2 & 1 & 2 & 1 & 2 & N/A & N/A & 4 & 6 \\ \midrule

DMC~\cite{decker2015fast} & N/A & N/A & 2+d & 2(2+d) & 1 & 2 & N/A & N/A & 3+d & 2(3+d) \\ \midrule

TeeChain~\cite{lind2019teechain} & 1 & 1+$p$/2 & off chain & off chain & off chain & off chain & 1 & 1+$p$/2+$m$ & 2 & 2+$p$+$m$ \\ \midrule

SFMC~\cite{burchert2018scalable} & 1/$\aveChannel{}$ & p/$\aveChannel{}$ & off chain & off chain & off chain & off chain & 1/$\aveChannel{}$ & $p$/$\aveChannel{}$ & 2/$\aveChannel{}$ & 2$p$/$\aveChannel{}$ \\ \midrule

Speedster & 1/$\aveChannel{}$ & 1/$\aveChannel{}$ & off chain & off chain & off chain & off chain & 1/$\aveChannel{}$ & 1/$\aveChannel{}$ & 2/$\aveChannel{}$ & 2/$\aveChannel{}$ \\ \bottomrule

\end{tabular}
\end{table*}

==> paragraphs/figure/prot_channel.tex <==
\begin{figure}[htbp]
\begin{framed}
 
\begin{center}
  
\textbf{Prot}$_{channel}$
        
\end{center}

\noindent \textbf{On receive}('init', $R$, $ccid$, $cid$)

$Sent := 0, Recv := 0, Cert := \perp, r := 0$

$ck  \sample \mathcal{AE}.\kgen(\secparam)$;

% $ct$ := $\mathcal{AE}.Enc(ck,$'authenticate'$\parallel cert)$

return ($cert$)

\bigskip

\noindent \textbf{On receive}('authenticate', $R$, $cert$)

assert $ Cert = \perp$

parse $cert$ as ($msg,\sigma$)

$Cert := cert$ if $\Sigma.Vf(pk_R,msg,\sigma)$ is true

\bigskip

\noindent \textbf{On receive}('send', $R$, $ct$)% \$val, inp):

assert $Cert \neq \perp$

assert ($cmd,msg$) := $\mathcal{AE}.Dec(ck,ct)$ valid

parse $msg$ as ($\$val,inp$)

$Recv+= \$val$

$count+=1$

return($R$,$inp$)

\bigskip

\noindent \textbf{On receive}('send',$cmd$,$inp$)

$ct := \mathcal{AE}.Enc(ck,inp)$

return($cmd$,$ct$)

\bigskip

\noindent \textbf{On receive}('claim')

assert $Cert_{\neg b} \neq \perp$

$Recv_b+= \$val $

% send($Cert_{\neg b}, Recv_b$) to $\mathcal{P}_b$

\end{framed}
\caption{Protocol of certified Channel \textbf{Prot}$_{channel}$} 
\label{fig:Ideal_channel}
\end{figure}

==> paragraphs/figure/prot_enclave.tex <==
%%%%%%%%%%%%################################%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%################################################%%%%%%%%%%%%%%
% Implementation of TEE prog
%##################
%%%%%%%%%%%%%%%%%################################################################%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%################################################################%%%%%%%%%%%%%%%%%%
\begin{figure*}[htbp]
% \vspace{-36pt}
\begin{center}
  \textbf{Protocol} $\Pi_{\TheName{}}(\idealP{}_{\mathcolor{0}}, \idealP{}_{\mathcolor{1}}, \idealP{}_{\mathcolor{2}}, ... ,\idealP{}_{\mathcolor{N}}]$
\end{center}
\begin{framed}
\begin{flushleft}

\begin{center}
Program \prog{}
\end{center}

\begin{multicols}{2}

\noindent \textbf{Initially:}

\sffont{bal} := $\emptyset$,
\sffont{certs} := $\emptyset$,
\sffont{channels} := $\emptyset$,
\spstate$^0$ := $\perp$

\bigskip

\setlength\parindent{15pt}

\noindent \colorgray{(1)} \textbf{On receive}(``init")

$(\pk,\sk) \sample \kgen(\secparam)$

% $\sigma_{att} := \Sigma.\sig(\msk,(\prog{}, \pk, \spstate^0))$
$\mpk := \mathcal{G}_{att}$.getpk()

\textbf{return} ($\pk, \mpk$)

\bigskip

\noindent \colorgray{(2)} \textbf{On receive} (``deposit", \tx)

parse \tx{} as (\_, \pk', \$val, $\sigma$)

assert \spstate$^0$ $\neq \perp$  and \$val $\geq 0$

assert $\sffont{Verify} (\pk, \tx, \sigma)$ is true

\sffont{bal} += \$val; assign (\tx, \$val) to \spstate$^0$
% leak ('deposit', $\\tx{}) to $\adv$

\bigskip

\noindent \colorgray{(3)} \textbf{On receive} (``open", \cid, $\idealR{}$, \inp)

$\ccid := \hash(SORT\{\pk_{\idealR{}}, \pk\})$

abort if \sffont{channels}[\ccid] $\neq \perp$ 

$\ck \sample \bin^*$ \texttt{// channel key}

$\cp{} := \{\pk, \pk_{\idealR{}}\}$

(\sffont{st}, \outp{}) := Contract$_{\cid{}}(\sk{}, \text{\sffont{bal}}, \overrightarrow{0}, \cp{})$

append ($\ccid, (\ck, \cid, \sffont{st}, \cp)$) to \sffont{channels}

$\sigma = \sffont{sign} (\sk, {\pk}_R\concat \inp)$, 
\cert{} = $(\pk\concat \pk_R\concat \inp\concat \sigma)$

% $\sigma_{att}$ := \sffont{Sign} (\msk, (\prog{}, \pk, $\spstate^0$))

\textbf{return} (\cert, \spstate$^0$, \outp{})

\bigskip

\noindent \colorgray{(4)} \textbf{On receive} (``openMulti", \cid, \{\ccid\}$^*$) 

for each $\ccid' \in \{\ccid\}^*$:
\setlength\parindent{25pt}

assert \sffont{channels}[$\ccid'$] $\neq \perp$

extract $\pk{}'$ from \sffont{channels}[$\ccid'$]

\setlength\parindent{15pt}

$\cp := \{\{ \pk'\}^*\cup\pk\}$; $\ccid{} := \hash(SORT(\cp))$

assert \sffont{channels}[\ccid] = $\perp$

$\sffont{gk} \sample \bin^*$ \texttt{//Group key}

(\sffont{st}, \outp) := Contract$_{\cid}(\sk_i, \spstate, \overrightarrow{0}, \cp)$

append ($\ccid, (\sffont{gk}, \cid, \sffont{st}, \cp)$) to \sffont{channels}

\ct{} := \sffont{Enc} (\sffont{gk}, \outp{})

\textbf{return} (\ct{})

\bigskip

\noindent \colorgray{(5)} \textbf{On receive} (``authenticate", \ccid, \idealR{}, \cert)

abort if \sffont{certs}[\ccid][\pk$_{\idealR{}}$] $\neq \perp$

parse \cert{} as ($\msg,\sigma$)

assert \sffont{Verify} $(\pk_{\idealR{}}, \msg, \sigma)$

set \sffont{certs}[\ccid][\pk$_{\idealR{}}$] to \cert

% \textbf{return} (\cert{})

\bigskip

\noindent \colorgray{(6)} \textbf{On receive} (``send", \ccid, \inp):

assert \sffont{certs}[b] $\neq \perp$

(\ck, \cid, \sffont{st}, \cp) := channles[\ccid]

(\sffont{st\'}, \outp{}) := Contract$_{\cid}(\sk, \spstate, \sffont{st}, \inp)$

update \sffont{channels}[\ccid] to (\ck, \cid, \sffont{st\'}, \cp)

\msg{} := (\pk\concat \inp\concat \sffont{st}'\concat \outp);
\ct{} := \sffont{Enc} (\ck, \msg) 

\textbf{return} (\ct)

\bigskip

\noindent \colorgray{(7)} \textbf{On receive} (``claim")

freeze \textbf{send} function

\tx{} := \{\cert\}$^*$\concat\spstate; $\sigma$ := \sffont{Sign} (\sk,\tx)

\textbf{return} (\tx\concat$\sigma$)

% \noindent \textbf{On receive}('dispute',$\idealR{}$)

% \textbf{return}()
\end{multicols}

\end{flushleft}
\end{framed}


\caption{\prog{} program of $\Pi_{\TheName{}}$} 
\label{fig:prog_TEE}
\end{figure*}

==> paragraphs/figure/prot_mux.tex <==
\begin{figure}[htbp]

\begin{center}
  \textbf{Protocol} $\Pi_{\TheName{}}(\idealP{}_{\mathcolor{0}}, \idealP{}_{\mathcolor{1}}, \idealP{}_{\mathcolor{2}}, ... ,\idealP{}_{\mathcolor{N}}]$
\end{center}
\begin{framed}
\vspace{-8pt}
\begin{center}

Program \mux{}

\end{center}
\setlength\parindent{5pt}
\noindent \textbf{Initially:}

$//$ \texttt{abstract out the sid}

\eid{} := \idealGatt{}.install (\prog{})

(\pk{}, \mpk{}) := \idealGatt{}.resume (``init")

make (\pk{}, \mpk{}) public

\bigskip

\noindent\textbf{Receive}(\tx{}) from the environment \idealE{}: 

parse \tx{} as (\pk{}, \ccid{}, \ct{}), abort if $\perp$

% assert $\Sigma.\verify(\pk, params,\sigma)$

\outp{} := \idealGatt{}.resume (\eid, \ccid, \ct, \sffont{switch} := \sffont{off})

\textbf{return} \outp{}

\bigskip

\noindent\textbf{Send} (\ccid{}, \inp{}) 

parse \inp{} as (\sffont{cmd}, \sffont{params})

% assert $\Sigma.\verify(\pk, params, \sigma)$

if \sffont{cmd} is ``open":

\setlength\parindent{15pt}

(\cert, \state$^0$, \outp{}, $\sigma_{att}$) := \idealGatt{}.resume(\eid, \ccid, \inp)

send \cert{} to counterpart if attestation passes
\setlength\parindent{5pt}

otherwise:
\setlength\parindent{15pt}

\outp{} := \idealGatt{}.resume (\eid, \ccid, \inp{}, \sffont{switch} := \sffont{off})


send (\ccid, \outp{}) as \tx{} to each \idealP{} in channel \ccid{}

% \bigskip

% \noindent\textbf{Claim}($R$) 

% % assert $\Sigma.\verify(\pk, params, \sigma)$

% ($\{cert,\$val\}, \sigma$) :=$\idealGatt{}$.resume($eid$, $R$, $\perp$ 'claim')

% Send ($\{cert,\$val\}, \sigma$) as $tx$ to $\mathcal{F}_{blockchain}$

\end{framed}
\caption{The \mux{} module of \protSpeedster{}{}} 
\label{fig:prog_mux}
\end{figure}
